Network-Clustered Multi-Modal Bug Localization

Developers often spend much effort and resources to debug a program. To help the developers debug, numerous information retrieval (IR)-based and spectrum-based bug localization techniques have been devised. IR-based techniques process textual information in bug reports, while spectrum-based techniques process program spectra (i.e., a record of which program elements are executed for each test case). While both techniques ultimately generate a ranked list of program elements that likely contain a bug, they only consider one source of information--either bug reports or program spectra--which is not optimal. In light of this deficiency, this paper presents a new approach dubbed Network-clustered Multi-modal Bug Localization (NetML), which utilizes multi-modal information from both bug reports and program spectra to localize bugs. NetML facilitates an effective bug localization by carrying out a joint optimization of bug localization error and clustering of both bug reports and program elements (i.e., methods). The clustering is achieved through the incorporation of network Lasso regularization, which incentivizes the model parameters of similar bug reports and similar program elements to be close together. To estimate the model parameters of both bug reports and methods, NetML employs an adaptive learning procedure based on Newton method that updates the parameters on a per-feature basis. Extensive experiments on 355 real bugs from seven software systems have been conducted to benchmark NetML against various state-of-the-art localization methods. The results show that NetML surpasses the best-performing baseline by 31.82%, 22.35%, 19.72%, and 19.24%, in terms of the number of bugs successfully localized when a developer inspects the top 1, 5, and 10 methods and Mean Average Precision (MAP), respectively.

==> approach.tex <==
\subsection{Overview}
\begin{figure}[t]
\center
\caption{Overal Framework (TF-IDF stands for weights of {Term Frequency\textendash Inverse Document Frequency})}
\includegraphics[scale=0.55,angle=-90]{framework_0001.eps}
\label{fig:framework}
\end{figure}

Fig. \ref{fig:framework} demonstrates the overall framework of our proposed approach. In the figure, our approach takes as input a set of program methods from a target program, a bug report extracted from a bug tracking system (e.g., Jira, or Bugzilla), and a set of valid test cases. Among the input test cases, there must be at least one test case that the target program returns an unexpected result (i.e., failed test cases). With the above input, we extract program methods from source code units to create a corpus of documents, and conduct text preprocessing step to remove some special symbols, and normalize terms to improve bug localization accuracy. After text preprocessing, we calculate \textit{td\textemdash idf} weights of words in input documents (i.e., program methods) (Section \ref{sec:bug_localization}).  On the other hand, we instrument the target program, and execute input test cases to obtain program spectra (Section \ref{sec:sbfl}). Importantly, for each of test cases, we not only pay attention to executed program methods or files, but we also record executed words during the execution of a test cases. In our approach, we value the importance of suspicousness scores at program method level, and especially word level, as if a document contains highly suspicious words according to the execution of test cases, it is more likely to be faulty. Finally, we combine obtained \textit{tf\textemdash idf} weights, and suspicousness scores into Vector Space Model in order to capture valuable information from input bug reports, and test cases to localize faulty program methods. The following sections describe details of components in Fig. \ref{fig:framework}.

\subsection{Method Corpus Creation \& Text Preprocessing}


\subsection{Recording Program Spectra}\label{sec:record_spectra}


\subsection{Combining TF-IDF weighting and Word-based Suspiciousness Scores}\label{sec:sstfidf}

In this section, we define a new statistic that combine \textit{TF-IDF} weighting the suspiciousness scores of words. We denote the statistic as \textit{SSTFIDF} which stands for Suspiciousness Score\textendash Term Frequency\textendash Inverse Document Frequency. Given a word $w$ in a document $d$ of a method corpus $C$, the following is the formula of word $w$:
\begin{equation}
SSTFIDF(w,d,C)=SS_{word}(w)\times \textit{TF-IDF}(w,d,C)
\label{eq:sstfidf}
\end{equation}


In the above formula, $SS_{word}(w)$ is the suspiciousness score of word $w$ returned by a particular spectrum-based fault localization formula using the collected raw statistics (Section \ref{sec:record_spectra}), and $\textit{TF-IDF}(w,d,C)$ is the Term Frequency\textendash Inverse Document Frequency of word $w$ in document $d$ of corpus $C$. According to the formula, our proposed \textit{SSTFIDF} is the extension of \textit{TF-IDF} which takes into account the suspiciousness aspect of a word in a document. The purpose of $SS_{word}$ in our formula is that it helps assign higher weights to words that have higher suspiciousness scores. In particular, if a word has a higher suspiciosuness score, the program elements containing the word are likely to be faulty, as SBFL raw statistics of words are collected according to their containing program elements (i.e.,statements, basic blocks, methods, classes). On the other hand, words with very low or zero suspiciousness scores are likely to be least relevant to under-consideration bugs. Hence, our \textit{SSTFIDF} also helps exclude such cases when words with high \textit{TF-IDF} weights, but actually not relevant to the bugs mentioned in the bug report, and addressed by the input set of test cases.


%In our paper, we calculate $TF(w,d)$, and $IDF(w,C)$ using Equation \ref{eq:tfidf} in Section \ref{sec:bug_localization}. Therefore, the following is the detailed formula of \textit{SSTFIDF} of word $w$ in document $d$ in corpus $C$ used in our experiments:
%\begin{align*}
%SSTFIDF(w,d,C)=&SS_{word}(w)\times \log(f(w,d)+1)\\
%&\times \log\frac{|C|}{|{d_i\in C : w \in d_i }|}
%\end{align*}

%The  measure is built upon the well-known statistic Term Frequency\textendash Inverse Document Frequency (TF\textendash IDF).

\subsection{Text Retrieval Model using Suspiciousness Scores}

%method suspiciousness scores

%VSM
%SSTFIDF
%value method tarantula scores

%weighted sum

\subsubsection{Proposed Model}

In this section, we propose the text retrieval model that combines \textit{TF-IDF} weighting with word-based, and method-based suspiciousness scores. The purpose of the combination is to maximize the ranking of relevant documents (i.e., faulty methods). Our approach is built upon the standard text retrieval model\textemdash Vector Space Model (VSM) with the utilization of suspiciousness scores. We denote our approach as $VSM^{susp}$. Similar to standard VSM, $VSM^{susp}$ represents each document as a vector of weights where each weight corresponds to a word. In $VSM^{susp}$, we compute the weight of each word using $SSTFIDF$ statistic (Section \ref{sec:sstfidf}). Following Equation  \ref{eq:sstfidf}, the weight of word $w$ in document $d$ of corpus $C$ is calculated as follows
\begin{align*}
SSTFIDF(w,d,C)&=SS_{word}(w)\times \log(f(w,d)+1)\\
&\times \log\frac{|C|}{|{d_i\in C : w \in d_i }|}
\end{align*}
In the above formula, $SS_{word}(w)$ is the suspiciousness score of word $w$ calculated by a generic spectrum-based fault localization formula, $f(w,d)$ is the number of times word $w$ appears in document $d$, and $d_i \in C$ means document $d_i$ is in set of document $C$. Similarly, $w \in d_i$ means word $w$ belongs to document $d_i$.

Given a bug report $q$, and document $d$ in method corpus, we compare the two documents by calculating the cosine similarity their document vector $\vec{q}$ and $\vec{d}$. We denote the cosine similarity between bug report $q$, and document $d$ in method corpus $C$ as $cosine(q,d,C)$. With the use of proposed statistic $SSTFIDF$, the value of $cosine(q,d,C)$ reflects the textual similarity between suspicious parts of bug report $q$, and document $d$ that contain suspicious words. However, there are still cases that documents with low or zero method-based suspiciousness scores still have high cosine similarity to the bug report. The reason is that documents in these cases are sharing suspicious words with the input bug report. Therefore, we multiply the cosine similarity by the suspiciousness scores of the document(i.e., method) to diminish ranking of irrelevant documents as well as increase ranking of . The following is the formula of the similarity between bug report $q$, and document $d$ in our proposed model:
\begin{align}
&sim_{VSM}^{susp}(q,d,C)=SS_{method}(d)\nonumber \\
&\times \frac{\sum\limits_{w\in q \cap d} SSTFIDF(w,q,C)\times SSTFIDF(w,d,C)}{\sqrt{\sum\limits_{w \in q} SSTFIDF(w,q,C)^2} \times \sqrt{\sum\limits_{w \in d} SSTFIDF(w,d,C)^2}}
\label{eq:sum_vsm_susp}
\end{align}

In the above formula, $SS_{method}(d)$ is method-based suspiciousness scores of document $d$ calculated by a spectrum-based fault localization formula, and $SSTFIDF(w,d,C)$ is the Suspiciousness Score\textendash Term Frequency\textendash Inverse Document Frequency statistic of word $w$ in document $d$ of corpus $C$ (Section \ref{sec:sstfidf}).

\subsubsection{Instance-based Composite Model}\label{sec:composite_model}

We propose a model that combines our proposed $VSM^{susp}$, standard VSM, and spectrum-based fault localization together to create a powerful composite bug localization model.  The formula of similarity score between bug report $q$, and document $d$ is as follows
\begin{align}
sim_{comp}&(q,d,C)=\alpha \times SS_{method}(d)+\beta \times sim_{VSM}^{susp}(q,d,C) \nonumber\\
&+ (1-\alpha-\beta) \times sim_{VSM}^{std}(q,d,C)
\label{eq:composite}
\end{align}
%(0 \leq \alpha, \beta \leq 1)
In the above formula, $SS_{method}(d)$ is the method-based suspiciousness scores of $d$ estimated by a spectrum-based fault localization, $sim_{VSM}^{susp}(q,d,C)$ is the similarity score between $q$, and $d$ output by our proposed $VSM^{susp}$ model (Equation \ref{eq:sum_vsm_susp}), $sim_{VSM}^{std}$ is the cosine similarity between of $q$, and $d$ in the standard Vector Space Model, $\alpha$ and $\beta$ are two constants in range of $[0..1]$. In our composite model, each member score has got a coefficient to determine how much its corresponding model contributes to the composite similarity score. With an appropriate combination of $\alpha$, and $\beta$, the composite model can smooth some of retrieval noise from its member models to achieve the best performance. Importantly, instead of using the same pair of $\alpha$, and $\beta$ for all the bug reports, we customize values of $\alpha$, and $\beta$ for every single bug report. We use information of similar known bug reports to estimate $\alpha$, and $\beta$. Given an input bug report, we first retrieve the top $K$ similar known bug reports to the input bug report  using standard Vector Space Model. Then, we infer the best pair of $\alpha$, and $\beta$ among the these $K$ bugs. The inferred values of $\alpha$, and $\beta$ are used to compute the similarity scores of documents using Equation \ref{eq:composite}. Overall, our proposed composite retrieval model tries to capture the specific property of each input bug report. Therefore, we refer to our composite model as instance-based composite model.


% For each input bug report, we customize the values of $\alpha$, and $\beta$ using information of similar bugs to maximize the performance of bug localization.


%\subsection{Retrieval Model}



==> body.tex <==

\section{Introduction}\label{sec.intro}
\input{intro}

\section{Background}\label{sec.prelim}
\input{prelim}

\section{Proposed Approach}\label{sec.approach}
\input{approach-2}

\section{Experiments }\label{sec.exp}
\input{exp}

\section{Related Work}\label{sec.related}
\input{related}

\section{Conclusion and Future Work} \label{sec.conclusion}
\input{conclusion}

%\section{Acknowledgment}
%\input{acknowlegement} 

==> discussion.tex <==
discussion

==> extension.tex <==
%\recheck{Richard: May you read this section to see whether my explanation is correct? Thank you :)}
%
%\recheck{Richard: Please let's me know whether section 3.2 and 3.3 are consistent.}

As we mention in Section~\ref{sec.intro}, \underline{A}daptive \underline{M}ulti-modal bug \underline{L}ocalization (AML)~\cite{Le:2015:IRS:2786805.2786880} remains two main issues. Firstly, AML only proposes the concept of model parameter for bug reports. In particular, every method $m$ share the same bug report parameter when estimating the suspiciousness scores of $m$, without considering the method parameter. Hence, AML may not capture the properties of different methods, leading to limit its effectiveness of detecting bug. Secondly, the  paprameter of each bug report is learned independently of other bug report, without exploiting the clustering and/or similarity properties of different bug reports and methods. In practice, some bug reports as well as methods are similar to other bug reports/methods. However, AML simply ignores the relationship between bug reports and methods. 

In light of these issues, we propose a new algorithm, namely \underline{N}etwork-clustered \underline{M}ulti-modal Bug \underline{L}ocalization (NetML). More specifically, NetML tries to addresses these two shortcomings by performing joint optimization of localization loss function and clustering of both bug reports and methods, and hence NetML involves two extensions. In this section, we focus on the first extension of NetML, trying to integrates two sets of model parameters (i.e., bug reports and methods) to localize bug more accurately. In particular, NetML redefine the suspiciousness score of method $m$ given by bug reports $b$ as an interaction between a bug report’s parameter vector $u_b$ and a method’s parameter vector $v_m$, as follows:

%The first is to redefine the suspiciousness score of method $m$ given by bug reports $b$ as an interaction between a bug report’s parameter vector $u_b$ and a method’s parameter vector $v_m$. In particular, NetML 
%We propose \underline{N}etwork-clustered \underline{M}ulti-modal Bug \underline{L}ocalization (NetML) that involves two extensions. The first is to redefine the suspiciousness score of method $m$ given by bug reports $b$ as an interaction between a bug report’s parameter vector $u_b$ and a method’s parameter vector $v_m$, as follows: 
%The first is to redefine the function of suspiciousness score (see equation \ref{eqn:composite}) as an interaction between a bug report’s parameter vector $u_b$ and a method’s parameter vector $v_m$, as follows:
\begin{align}
\label{eq:aml_plus}
f(x_{i}, u_b, v_m) & = \sum_{j = 1}^{J} (u_{b,j} + v_{m,j}) x_{i,j} \nonumber \\
& = \sum_{j = 1}^{J} u_{b,j} x_{i,j} + \sum_{j = 1}^{J} v_{m,j} x_{i,j}
\end{align}
where $x_i$ is denoted as feature vector of specific method $m$ given bug report $b$ and program spectra $p$ (i.e., $b, p, m$). $J$ is a number of features, hence $J = 3$ in our model since we only have three components NetML$^\text{Text}$, NetML$^\text{Spectra}$ and NetML$^\text{SuspWord}$ (see Figure~\ref{fig:framework}). Different to the original multi-modal technique (i.e., AML), each feature vector ($b, p, m$) not only considers the parameter of bug report $b$ but also share the parameter of method $m$.



%In light of these issues, we propose a new algorithm, namely \underline{N}etwork-clustered \underline{M}ulti-modal Bug \underline{L}ocalization (NetML). More specifically, NetML tries to addresses these two shortcomings by performing joint optimization of localization loss function and clustering of both bug reports and methods. Firstly, NetML integrates two sets of model parameters (i.e., bug reports and methods) to localize bug more accurately. Secondly, NetML takes advantage of network Lasso regularization~\cite{Hallac:2015:NLC:2783258.2783313} to enforce similar bug reports as well as methods to have similar model parameters. Thus, the proposed approaches may achieve a more effective bug localization. 
%
%In the following section, we firstly present a short introduction about network Lasso, and briefly explain our proposed algorithm, i.e., NetML. 
%
%
%%Firstly, for each bug report $b$, a fixed parameter vector $\vec{\theta}_b = (\alpha, \beta, \gamma)$ is inferred for all methods $m$ (see Equation~\ref{eqn:composite}). 
%%In other words, every method $m$ shares the same parameter vector $\vec{\theta}_b$ when estimating the suspiciousness scores of $m$ according to bug report $b$ and program spectra $p$. In particular, each method $m$ not only considers the parameter of bug report $b$ but also share the parameter of method $m$. 
%%Therefore, Equation~\ref{eqn:composite} does not accurately reflect the suspiciousness score of method $m$ given bug report $b$ and program spectra $p$. Secondly, the parameter vector $\vec{\theta}_b$ of a bug report is learned independently of other bug report $b'$, without exploiting the clustering and/or similarity properties of different bug reports and methods. In practice, some bug reports as well as methods are similar to other bug reports/methods. However, the instance-wise loss function in equation \ref{eq:instance-wise-loss} ignores the relationship between the bug reports and the methods. In light of these issues, we proposed a new algorithm, namely generalized adaptive multi-modal bug localization, to tackle these problems in bug localization. 
%
%%Our proposed algorithm is inspired by network lasso \cite{Hallac:2015:NLC:2783258.2783313}. In the next sub section, I briefly present a short introduction about network lasso, then explain the proposed algorithm, i.e. \underline{G}eneralized \underline{A}daptive \underline{M}ulti-modal bug \underline{L}ocalization (AML*).
%
%\subsubsection{Network Lasso}\label{subsec:networklasso}
%
%Nowadays, convex optimization has become a popular way of modeling problems in many different fields (i.e., clock synchronization, smart power grids, state estimation, etc.). However, classical methods of convex analysis, relying on interior point methods~\cite{Renegar:2001:MVI:502968}, begin to fail due to a lack of scalability since datasets is getting larger and more intricate. The challenge of large-scale optimization lies in developing methods general enough to work well independent of the input, while being capable of scaling to the immense datasets that today’s applications require. In~\cite{Hallac:2015:NLC:2783258.2783313}, Hallac et al. proposed a network setting, namely network Lasso, that allows for simultaneous clustering and optimization on graph. In particular, given a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the vertex set and $\mathcal{E}$ is the edges of graph. The network Lasso problem is defined as following: 
%
%%Therefore, it is necessary to formulate general classes of convex optimization solvers, ones that can apply to a variety of interesting and relevant problems, and to develop algorithms for reliable and efficient solutions.
%
%%Network Lasso~\cite{Hallac:2015:NLC:2783258.2783313} is a generalization of the group lasso to a network setting that allows for simultaneous clustering and optimization on graphs. In~\cite{Hallac:2015:NLC:2783258.2783313}, Hallac et al. focused on optimization problem posed on graph. Given a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the vertex set and $\mathcal{E}$ is the edges of graph. The network lasso problem is defined as following: 
%\begin{align}
%\label{eq:network_lasso}
%	minimize \sum_{i \in \mathcal{V}}^{} f_i(x_i) + \lambda \sum_{(j, k) \in \mathcal{E}}^{} w_{jk} \|x_j - x_k \|_{2}	
%\end{align}
%The variable are $x_1, \dots, x_n \in R^{p}$, where $n = |\mathcal{V}|$. $x_i \in R^{p}$ is the variable at node $i$, $f_i$ is the cost function at node $i$, $w_{jk}$ is the relative weights among the edges $(j,k)$ of the network $\mathcal{G}$, and $\lambda$ is an overall parameter that scales the edge objectives relative to the node objectives. In order to solve the problem \ref{eq:network_lasso} in a distributed and scalable manner, which allows for guaranteed global convergence even on large graphs, the author based on the Alternating Direction Method of Multipliers (ADMM)~\cite{Parikh:2014:PA:2693612.2693613, Boyd:2011:DOS:2185815.2185816}. With ADMM, each individual component solves its own private objective function, passes this solution to its neighbors, and repeats the process until the entire network converges. 

\subsection{Optimization Objective}
\label{subsec:extension}
%NetML takes advantage of network Lasso regularization~\cite{Hallac:2015:NLC:2783258.2783313} to enforce similar bug reports as well as methods to have similar model parameters
The second extension takes advantage of network Lasso regularization~\cite{Hallac:2015:NLC:2783258.2783313} to enforce similar bug reports as well as methods to have similar model parameters. Different from the original network Lasso that only deals with a single graph, our approach involves optimizing over two graphs simultaneously. Specifically, we consider a joint optimization over the bug
similarity graph $\mathcal{G}^B=\{e_{b,b'}|(b, b') \in B\}$, and method similarity graph $\mathcal{G}^M=\{e_{m,m'}|(m, m') \in M\}$.

With the new model parameterization and similarity graphs taken into account, we propose a new dual network Lasso-regularized loss function as following:
\begin{align}
\label{eq:NL_lossfunc}
	\mathcal{L}_i & = -\sum_{b=1}^{B}\sum_{m=1}^{M} w_i \bigg[y_i log(\sigma(f(x_i, u_b, v_m))) \nonumber\\
	& + (1 - y_i) log(1- \sigma(f(x_i, u_b, v_m))) \bigg] \nonumber\\
	& + \frac{\alpha}{2} \sum_{j=1}^{J} \bigg[\sum_{b=1}^{n_{B}} u_{b,j}^2 + \sum_{m=1}^{n_{M}} v_{m,j}^2 \bigg] \nonumber\\
	& + \frac{\beta}{2} \sum_{j=1}^{J} \bigg[ \sum_{(b, b' \in \mathcal{G}^B)}^{} e_{b, b'} (u_{b,j} - u_{b', j})^2 \nonumber\\ 
	& + \sum_{(m, m' \in \mathcal{G}^M)}^{} e_{m, m'} (u_{m,j} - u_{m', j})^2 \bigg]
\end{align}
where $B$ and $M$ are the number of bug reports and methods in our dataset, $u_b$ and $v_m$ are called the parameter vector of bug reports and methods respectively, $y_i$ denotes the label of method $m$ given bug report $b$, $\sigma(x_i)$ is the logistic function \cite{Collins:2002:LRA:599615.599689}, $w_i$ used to automatically adjust weights inversely proportional to class frequencies in the training data. In NetML, $w_i$ is applied to solve the skewed distribution problem in bug localization task, i.e., the number of positive labels is much smaller than the number of negative labels. $\alpha$ and $\beta$ are the learning rate of regularization in our loss function. Intuitively, the implication of the network lasso regularization is straightforward—the more similar two bug reports (or two methods) are, the closer their parameter vectors (i.e., $u_b$ and $v_m$) should be. 

To minimize $\mathcal{L}_i$, we employ a Newton method \cite{doi:10.1137/1.9780898718898} stemming from a second-order Taylor series expansion of the loss function $\mathcal{L}_i$, which are defined as following:

\begin{align}
\label{eq:newton}
	\mathcal{L}_i(\theta) = \mathcal{L}_i(\theta_0) + \triangledown \mathcal{L}_i(\theta_0) (\theta - \theta_0) + \frac{\triangledown^2 \mathcal{L}(\theta_0)}{2} (\theta - \theta_0)^2
\end{align}

The minimal of $\mathcal{L}_i$ can be obtained by taking the (partial) derivative of $\mathcal{L}(\theta)$ and equating it to zero:
\begin{align}
0 &= \triangledown \mathcal{L}_i(\theta_0) + \triangledown^2 \mathcal{L}_i(\theta_0) (\theta - \theta_0) \nonumber\\
\theta &= \theta_0 - \frac{\triangledown \mathcal{L}_i(\theta_0)}{\triangledown^2 \mathcal{L}_i(\theta_0)}
\end{align}

If we take $\theta_0$ as the old estimate of $u_{b,j}$ or $v_{m,j}$, this leads to the following update procedures:
\begin{align}
\label{eqn:update_u}
u_{b,j} &\leftarrow u_{b,j} - \frac{ \triangledown \mathcal{L}_i(u_{b,j}) }{ \triangledown^2 \mathcal{L}_i(u_{b,j}) } \\
\label{eqn:update_v}
v_{m,j} &\leftarrow v_{m,j} - \frac{ \triangledown \mathcal{L}_i(v_{m,j}) }{ \triangledown^2 \mathcal{L}_i(v_{m,j}) }
\end{align}

In turn, we need to compute the first and second derivatives of each parameter $u_{b,j}$ and $v_{m,j}$. For the bug report parameter $u_{b,j}$, the first and second derivatives are respectively:
\begin{align}
\label{eqn:grad_u}
\triangledown \mathcal{L}_i(u_{b,j}) &= \sum_{m=1}^{n_{M}} \left[ w_{i} (\sigma(f(x_i, u_b, v_m)) - y_{i}) x_{i,j} \right] \nonumber \\
&+ \alpha u_{b,j} + \beta \sum_{b'} \left[ e_{b,b'} \left( u_{b,j} - u_{b',j} \right) \right] \\
\label{eqn:hess_u}
\triangledown^2 \mathcal{L}_i(u_{b,j}) &= \sum_{m=1}^{n_{M}} \left[ w_{i} \sigma(f(x_i, u_b, v_m)) ( 1 - \sigma_{i}) x_{i,j}^2 \right] \nonumber \\
&+ \alpha + \beta \sum_{b'} e_{b,b'}
\end{align}

Similarly, we can compute the first and second derivatives w.r.t each method parameter $v_{m,j}$ as:
\begin{align}
\label{eqn:grad_v}
\triangledown \mathcal{L}_i(v_{m,j}) &= \sum_{b=1}^{n_{B}} \left[ w_{i} (\sigma(f(x_i, u_b, v_m)) - y_{i}) x_{i,j} \right] \nonumber \\
& + \alpha v_{m,j} + \beta \sum_{m'} \left[ e_{m,m'} \left( v_{m,j} - v_{m',j} \right) \right] \\
\label{eqn:hess_v}
\triangledown^2 \mathcal{L}_i(v_{m,j}) &= \sum_{b=1}^{n_{B}} \left[ w_{b,m} \sigma_{b,m} ( 1 - \sigma_{b,m}) x_{i,j}^2 \right] \nonumber \\
& + \alpha + \beta \sum_{m'} e_{m,m'}
% \label{eqn:grad_v}
% \triangledown \mathcal{L}(v_{m,j}) &= \sum_{b=1}^{n_{B}} \left[ (\sigma_{b,m} - y_{b,m}) u_{b,j} x_{b,m,j} \right] + \alpha v_{m,j} + \beta \sum_{m'} \left[ e_{m,m'} \left( v_{m,j} - v_{m',j} \right) \right] \\
% \label{eqn:hess_v}
% \triangledown^2 \mathcal{L}(v_{m,j}) &= \sum_{b=1}^{n_{B}} \left[ \sigma_{b,m} ( 1 - \sigma_{b,m}) u_{b,j}^2 x_{b,m,j}^2 \right] + \alpha + \beta \sum_{m'} e_{m,m'}
\end{align}

Finally, the update formula for $u_{b,j}$ can be obtained by substituting equation \ref{eqn:grad_u} and \ref{eqn:hess_u} into equation \ref{eqn:update_u}. Likewise, by substituting equation \ref{eqn:grad_v} and \ref{eqn:hess_v} into \ref{eqn:update_v} to update formula $v_{m,j}$. To learn the model parameters, we use a \emph{Newton method} that updates the parameters on a per-feature $j$ basis.
%Starting from a random initial values of $u_{b,j}$ and $v_{m,j}$, we first update $u_{b,j}$ by assuming that all $v_{m,j}$ are fixed. We then alternate by updating $v_{m,j}$ with all $u_{b,j}$ assumed to be fixed.

\subsection{Learning Procedure}
\label{sec:learning}

\begin{algorithm*}[!t]
	\begin{algorithmic}[1]
		\Require Matrix $X \in \mathbb{R}^{B \times M \times 3}$, where $B$ and $M$ are the number of bug reports and methods in our training data. Each cell in 3-D matrix is a vector $x_{b,m} = [\text{NetML}^{\text{Text}}(b,m), \text{NetML}^{\text{Spectra}}(p,m), \text{NetML}^{\text{SuspWord}}(b,p,m)]$ for given bug report $b$, program spectra $p$, and method $m$, label vector $y \in \mathbb{R}^{B \times M}$ (each element $y_{b, m}$ is the label of $x_{b, m}$), sample weight $w \in \mathbb{R}^{B \times M}$, learning rate $\eta$, regularization parameter $\alpha$ and $\beta$, maximum training iterations $T_{max}$
		\Ensure Weight parameters $U \in \mathbb{R}^{B \times 3}$ and $ V \in \mathbb{R}^{M \times 3}$ 
		\State Initialize all parameters $u_{b,j} \leftarrow 0$ and $v_{m,j} \leftarrow 0$
		\State Precompute constant terms $q_b \leftarrow \sum_{b'} e_{b,b'}$ and $q_m \leftarrow \sum_{m'} e_{m,m'}$
		\State Set the initial learning rate $\eta \leftarrow 1$
		\Repeat 
		\State Compute all predictions $\sigma(f(x_{b,m}, u_b, v_m))$ (see equation \ref{eq:aml_plus})
		\State $\mathcal{L}_{prev} \leftarrow -\sum_{b} \sum_{m} w_{b,m} \big[ y_{b,m} \log \big( \sigma(f(x_{b,m}, u_b, v_m)) \big) + \big( 1 - y_{b,m} \big) \log \big(1 - \sigma(f(x_{b,m}, u_b, v_m)) \big) \big]$
		\For {each $j \in \{ 1,\ldots,3 \}$}
		\State \textbf{/* Update all $u_{b,j}$ */}
		\For {each $b \in \{ 1,\ldots,B \}$}
		\State $p_{b} \leftarrow \sum_{b'} e_{b,b'} u_{b',j}$
		\EndFor
		\For {each $b \in \{ 1,\ldots,B \}$}
		\State $b_{num} \leftarrow \sum_{m=1}^{M} \big[ w_{b,m} (\sigma(f(x_{b,m}, u_b, v_m)) - y_{b,m}) x_{b,m,j} \big] + \beta \big[ u_{b,j} q_b - p_{b} \big] + \alpha u_{b,j}$
		\State $b_{deno} \leftarrow \sum_{m=1}^{M} \big[ w_{b,m} \sigma(f(x_{b,m}, u_b, v_m)) (1 - \sigma(f(x_{b,m}, u_b, v_m)) x_{b,m,j}^2 \big] + \beta q_b + \alpha$
		\State $u_{b,j} \leftarrow u_{b,j} - \eta \left( \frac{b_{num}}{b_{deno}} \right)$
		\EndFor
		
		\State \textbf{/* Update all $v_{m,j}$ */}
		\For {each $m \in \{ 1,\ldots,M \}$}
		\State $p_{m} \leftarrow \sum_{m'} e_{m,m'} v_{m',j}$
		\EndFor
		
		\For {each $m \in \{ 1,\ldots,M \}$}
		\State $v_{num} \leftarrow \sum_{b=1}^{B} \big[ w_{b,m} (\sigma(f(x_{b,m}, u_b, v_m)) - y_{b,m}) x_{b,m,j} \big] + \beta \big[ v_{m,j} q_m - p_{m} \big] + \alpha v_{m,j}$
		\State $v_{deno} \leftarrow \sum_{b=1}^{B} \big[ w_{b,m} \sigma(f(x_{b,m}, u_b, v_m)) (1 - \sigma(f(x_{b,m}, u_b, v_m))) x_{b,m,j}^2 \big] + \beta q_m + \alpha$
		\State $v_{m,j} \leftarrow v_{m,j} - \eta \left( \frac{v_{num}}{v_{deno}} \right)$
		\EndFor
		\EndFor
		\State Compute all predictions $\sigma(f(x_{b,m}, u_b, v_m)$
		\State $\mathcal{L}_{curr} \leftarrow -\sum_{b} \sum_{m} w_{b,m} \big[ y_{b,m} \log \big( \sigma(f(x_{b,m}, u_b, v_m)) \big) + \big( 1 - y_{b,m} \big) \log \big(1 - \sigma(f(x_{b,m}, u_b, v_m)) \big) \big]$
		\State $\eta \leftarrow
		\begin{cases}
		\frac{\eta}{2},   & \text{if } \mathcal{L}_{curr} > \mathcal{L}_{prev}\\
		\min(1, 2 \eta),  & \text{otherwise}
		\end{cases}$
		\Until $T_{max}$ iterations
	\end{algorithmic}
	\caption{Parameters learning for generalized adaptive multi-modal bug localization}
	\label{alg:network_lasso}
\end{algorithm*}

\begin{algorithm}
	\begin{algorithmic}[1]
		\Require Matrix $X \in \mathbb{R}^{B \times M \times 3}$, where $B$ and $M$ are the number of bug reports and methods in our training data. Bug reports graph $\mathcal{G}^B=\{e_{b,b'}|(b, b') \in B\}$, , where $e_{b,b'}$ represents textual similarity between $b$ and $b'$.
		\State folds $\leftarrow$ cross\_validation($\mathcal{G}^B.vertex$)
		\For {\textit{test} in folds}
		\State $B_{test}$ $\leftarrow$ $\mathcal{G}^B[test]$
		\For {each $b \in B_{test}$ }
		\State Finding top-K most similarity bug reports of $b$
		\State Construct matrix $X_{train} \in {B_{topK} \times M \times 3}$
		\State Calling Algorithm~\ref{alg:network_lasso} for matrix $X_{train}$ with default parameters
		\State Predict all methods given by particular bug report $b$ 
		\EndFor 
		\EndFor
	\end{algorithmic}
	\caption{Prediction procedure for localize bug report}
	\label{alg:prediction}
\end{algorithm}

Algorithm \ref{alg:network_lasso} summarizes our learning procedure to localize bug reports. For each feature component, NetML includes two basic steps: we first update bug report parameter vector (see step 8 of algorithm \ref{alg:network_lasso}) by applying equation~\ref{eqn:update_u}, and then update method parameter vector (in step 17) by employing equation~\ref{eqn:update_v}. For computational efficiency, we precompute the constant terms $q_b = \sum_{b'} e_{b,b'}$ and $q_m = \sum_{m'} e_{m,m'}$ before the Newton iterations begins. During each Newton iteration, we also calculate the terms $\sum_{b'} e_{b,b'} u_{b',j}$ and $\sum_{m'} e_{m,m'} v_{m',j}$ for each feature $j$.

To predict method $m$ given by a new bug report $b$ and program spectra $p$, we base on a set of top-K historical fixed bugs in a training data that are the most similar to $b$. We find these top-K nearest neighbors by measuring the textual similarity of $b$ with training (historical) bug reports using the vector space model. These top-K nearest neighbors are used to construct our NetML model. Note that the prediction steps are similar to~\cite{Le:2015:IRS:2786805.2786880}.

In step 4 of Algorithm~\ref{alg:network_lasso}, we repeat maximum training iterations until $T_{max}$. For each feature $j$ component in each iteration (see step 7), we update the bug report and method parameters across all bug reports $B$ and methods $M$ (in step 12 and step 21). Moreover, given a new bug report $b$, we only select top-K nearest neighbors that are most similar to $b$. Hence, time complexity of our proposed algorithm is $\text{O}(T_{max} \times Btest \times J \times (K + M))$, where $Btest$ is the number of bug reports in testing data, and $J$ is the number of features in our algorithm, thus $J = 3$ as we only have three feature components (i.e., $\text{NetML}^{\text{Text}}, \text{NetML}^{\text{Spectra}}, \text{NetML}^{\text{SuspWord}}$). Based on the time complexity, the space complexity of our proposed algorithm should be $\text{O}(Btest \times J \times (K + M))$ by discarding the number of iteration $T_{max}$.

\recheck{@Richard: please take a look at this section to see whether we need further clarification}

\subsection{Feature Engineering}\label{subsec:both}

NetML$^\text{Spectra}$ processes only the program spectra information using a spectrum-based bug localization technique described in Section~\ref{sec.prelim}. NetML$^\text{Spectra}$ in the end outputs a score for each method in the corpus. Given a program spectra $p$ and a method $m$ in a corpus $C$, NetML$^\text{Spectra}$ outputs a score that indicates how suspicious is $m$ considering $p$ which is denoted as NetML$^\text{Spectra}(p,m,C)$. By default, NetML$^\text{Spectra}$ uses Tarantula as the spectrum-based bug localization technique.

NetML$^\text{SuspWord}$ processes both bug reports and program spectra, and computes the suspiciousness scores of words to rank methods. Given a bug report $b$, a program spectra $p$, and a method $m$ in a corpus $C$, NetML$^\text{SuspWord}$ outputs a score that indicates how suspicious is $m$ considering $b$ and $p$; this is denoted as NetML$^\text{SuspWord}(b,p,m,C)$. 

The NetML$^\text{Integrator}$ component combines the NetML$^\text{Text}$, NetML$^\text{Spectra}$, NetML$^\text{SuspWord}$ components to produce the final ranked list of methods. Given a bug report $b$, a program spectra $p$, and a method $m$ in a corpus $C$, the adaptive integrator component outputs a suspiciousness score for method $m$ which is denoted as AML$(b,p,m,C)$.

The NetML$^\text{Text}$ and NetML$^\text{Spectra}$  components reuse techniques proposed in prior works which are described in Section~\ref{sec.prelim}. In the next subsections, we briefly describe the components namely NetML$^\text{SuspWord}$ and the network-clustered integrator component.

Parnin and Orso {highlighted} that ``future research could also investigate ways to automatically suggest or highlight terms that might be related to a failure''~\cite{ParninO11}, however they did not propose a concrete solution. We use Parnin and Orso's observation, which highlights that some words are indicative to the location of a bug, as a starting point to design our NetML$^\text{SuspWord}$ component. \iffalse NetML$^\text{SuspWord}$ component is designed based on this observation made by Parnin and Orso which highlights that some words are indicative to the location of a bug.\fi
This component breaks down a method into its constituent words, computes the suspiciousness scores of these words, and composes these scores back to result in the suspiciousness score of the method. The process is analogous to a machine learning or classification algorithm that breaks a data point into its constituent features, assign weights or importance to these features, and use these features, especially important ones, to assign likelihood scores to the data point. The component works in three steps: mapping of methods to words, computing word suspiciousness, and composing word suspiciousness into method suspiciousness. We describe each of these steps in the following sections. 

% component takes in a spectra and a bug report to compute the suspiciousness scores of words. The suspicious words are then used to rank methods. Different from the $AML^{SPECTRA}$ component that directly computes the suspiciousness scores of methods, this

\subsubsection{Mapping of Methods to Words}
In this step, we map a method to its constituent words. For every method, we extract the following textual contents including: (1) The name of the method, along with the names of its parameters, and identifiers contained in the method body; (2) The name of the class containing the method, and the package containing the class; (3) The comments that are associated to the method (e.g., the Javadoc comment of that method, and the comments that appear inside the method), and comments that appear in the class (containing the method) that are not associated to any particular method.

After we have extracted the above textual contents, we apply the text pre-processing step described in Section~\ref{sec.prelim}. At the end of this step, for every method we map it to a set of pre-processed words. Given a method $m$, we denote the set of words it contains as $words(m)$.

\subsubsection{Computing Word Suspiciousness}
We compute the suspiciousness score of a word by considering the program elements that contain the word. Let us denote the set of all failing execution traces in spectra $p$ as $p.F$ and the set of all successful execution traces as $p.S$. To compute the suspiciousness scores of a word $w$ given spectra $p$, we define several sets:
%\begin{eqnarray}
%EF(w,p) = \{t \in p.F | \exists {m\in t}~s.t.~w\in words(m)\}\footnotemark[1]\nonumber\\
%NF(w,p) = \{t \in p.F | \not\exists {m\in t}~s.t.~w\in words(m)\}\nonumber\\
%ES(w,p) = \{t \in p.S | \exists {m\in t}~s.t.~w\in words(m)\}\nonumber\\
%NS(w,p) = \{t \in p.S | \not\exists {m\in t}~s.t.~w\in words(m)\}\nonumber
%\end{eqnarray}
\begin{align*}
EF(w,p) &= \{t \in p.F | \exists {m\in t}~s.t.~w\in words(m)\}\nonumber\\
%NF(w,p) &= \{t \in p.F | \not\exists {m\in t}~s.t.~w\in words(m)\}\nonumber\\
ES(w,p) &= \{t \in p.S | \exists {m\in t}~s.t.~w\in words(m)\}\nonumber
%NS(w,p) &= \{t \in p.S | \not\exists {m\in t}~s.t.~w\in words(m)\}\nonumber
\end{align*}
The set $EF(w,p)$ is the set of execution traces in $p.F$ that contain a method in which the word $w$ appears. The set $ES(w,p)$ is the set of execution traces in $p.S$ that contain a method in which the word $w$ appears. Based on these sets, we can compute the suspiciousness score of a word $w$ using a formula similar to Tarantula as follows:
\begin{equation}
\text{SS}_{\text{word}}(w,p)=\frac{\frac{|EF(w,p)|}{|p.FAIL|}}{\frac{|EF(w,p)|}{|p.FAIL|}+\frac{|ES(w,p)|}{|p.SUCCESS|}}
\label{eq:ss}
\end{equation}

Using the above formula, words that appear more often in methods that are executed in failing execution traces are deemed to be more suspicious than those that appear less often in such methods.

%The set $NF(w,p)$ is the set of execution traces in $p.F$ that do not contain a method in which the word $w$ appears. The set $NS(w,p)$ is the set of execution traces in $p.S$ that do not contain a method in which the word $w$ appears.

\subsubsection{Computing Method Suspiciousness}
To compute a method $m$'s suspiciousness score, we compute the textual similarity between $m$ and the input bug report $b$, and consider the appearances of $m$ in the input program spectra $p$. In the textual similarity computation, the suspiciousness of words are used to determine their weights.

First, we create a vector of weights that represents a bug report and another vector of weights that represents a method. Each element in a vector corresponds to a word that appears in either the bug report or the method. The weight of a word $w$ in document (i.e., bug report or method) $d$ of method corpus $C$ considering program spectra $p$ is:
\begin{align*}
\text{SSTFIDF}(w,p,d,C)=&\text{SS}_{\text{word}}(w,p)\times \log(f(w,d)+1)\\
&\times \log\frac{|C|}{|{d_i\in C : w \in d_i }|}
\end{align*}
In the above formula, $\text{SS}_\text{word}(w,p)$ is the suspiciousness score of word $w$ computed by Equation~\ref{eq:ss}, $f(w,d)$ is the number of times word $w$ appears in document $d$, and $d_i \in C$ means document $d_i$ is in the set of document $C$. Similarly, $w \in d_i$ means word $w$ belongs to document $d_i$. The above formula considers the weight of a word based on its suspiciousness, and well-known information retrieval metrics: term frequency (i.e., $\log(f(w,d)+1)$) and inverse document frequency (i.e., $\log\frac{|C|}{|{d_i\in C : w \in d_i }|}$).

After the two vectors of weights of method $m$ and bug report $b$ are computed, we compute the suspiciousness score of the method $m$ by computing the cosine similarity of these two vectors multiplied by a weighting factor. The formula to compute this score is as follows:
\begin{align}
&\text{AML}^\text{SuspWord}(b,p,m,C)=\text{SS}_{\text{method}}(m,p)\nonumber \times\\
&\frac{\sum\limits_{w\in b \cap m} \text{SSTFIDF}(w,p,b,C)\times \text{SSTFIDF}(w,p,m,C)}{\sqrt{\sum\limits_{w \in b} \text{SSTFIDF}(w,p,b,C)^2} \times \sqrt{\sum\limits_{w \in m} \text{SSTFIDF}(w,p,m,C)^2}}
\label{eq:sum_vsm_susp}
\end{align}
Here we use $\text{SS}_\text{method}(m,p)$ that computes the suspiciousness score of method $m$ considering program spectra $p$ as the weighting factor. This can be computed by various spectrum-based bug localization tools. By default, we use the same fault localization tool as the one used in NetML$^\text{Spectra}$ component. With this, NetML$^\text{SuspWord}$ integrates both macro view of method suspiciousness (which considers direct execution of a method in the failing and correct execution traces) and micro view of method suspiciousness (which considers the executions of its constituent words in the execution traces).








==> method.tex <==

%In this section, we propose the text retrieval model that combines \textit{TF-IDF} weighting with word-based, and method-based suspiciousness scores. The purpose of the combination is to maximize the ranking of relevant documents (i.e., faulty methods). Our approach is built upon the standard text retrieval model\textemdash Vector Space Model (VSM) with the utilization of suspiciousness scores. We denote our approach as $VSM^{susp}$. Similar to standard VSM, $VSM^{susp}$ represents each document as a vector of weights where each weight corresponds to a word. In $VSM^{susp}$, we compute the weight of each word using $SSTFIDF$ statistic (Section \ref{sec:sstfidf}). Following Equation  \ref{eq:sstfidf}, the weight of word $w$ in document $d$ of corpus $C$ is calculated as follows
%\begin{align*}
%SSTFIDF(w,d)&=SS_{word}(w)\times \log(f(w,d)+1)\\
%&\times \log\frac{|C|}{|{d_i\in C : w \in d_i }|}
%\end{align*}
%In the above formula, $SS_{word}(w)$ is the suspiciousness score of word $w$ calculated by a generic spectrum-based fault localization formula, $f(w,d)$ is the number of times word $w$ appears in document $d$, and $d_i \in C$ means document $d_i$ is in set of document $C$. Similarly, $w \in d_i$ means word $w$ belongs to document $d_i$.
%
%Given a bug report $q$, and document $d$ in method corpus, we compare the two documents by calculating the cosine similarity their document vector $\vec{q}$ and $\vec{d}$. We denote the cosine similarity between bug report $q$, and document $d$ in method corpus $C$ as $cosine(q,d)$. With the use of proposed statistic $SSTFIDF$, the value of $cosine(q,d)$ reflects the textual similarity between suspicious parts of bug report $q$, and document $d$ that contain suspicious words. However, there are still cases that documents with low or zero method-based suspiciousness scores still have high cosine similarity to the bug report. The reason is that documents in these cases are sharing suspicious words with the input bug report. Therefore, we multiply the cosine similarity by the suspiciousness scores of the document(i.e., method) to diminish ranking of irrelevant documents as well as increase ranking of . The following is the formula of the similarity between bug report $q$, and document $d$ in our proposed model:
%\begin{align}
%&sim_{VSM}^{susp}(q,d)=SS_{method}(d)\nonumber \\
%&\times \frac{\sum\limits_{w\in q \cap d} SSTFIDF(w,q)\times SSTFIDF(w,d)}{\sqrt{\sum\limits_{w \in q} SSTFIDF(w,q)^2} \times \sqrt{\sum\limits_{w \in d} SSTFIDF(w,d)^2}}
%\label{eq:sum_vsm_susp}
%\end{align}
%
%In the above formula, $SS_{method}(d)$ is method-based suspiciousness scores of document $d$ calculated by a spectrum-based fault localization formula, and $SSTFIDF(w,d)$ is the Suspiciousness Score\textendash Term Frequency\textendash Inverse Document Frequency statistic of word $w$ in document $d$ of corpus $C$ (Section \ref{sec:sstfidf}).

The integrator component serves to combine the scores produced by the three components AML$^\text{Text}$, AML$^\text{Spectra}$ and AML$^\text{SuspWord}$ by taking a weighted sum of the scores. The final suspiciousness score of method $m$ given bug report $b$ and program spectra $p$ in a corpus $C$ is given by:
\begin{align}
\label{eqn:composite}
f(x_i, \theta) &= \alpha \times \text{AML}^\text{Text}(b,m) + \beta \times \text{AML}^\text{Spectra}(p,m) \nonumber\\
&+ \gamma \times \text{AML}^\text{SuspWord}(b,p,m)
\end{align}

\noindent where $i$ refers to a specific $(b,p,m)$ combination (aka \emph{data instance}), $x_i$ denotes the feature vector $x_i = [ \text{AML}^\text{Text}(b,m), \text{AML}^\text{Spectra}(p,m), \text{AML}^\text{SuspWord}(b,p,m)]$, and $\theta$ is the parameter vector $[ \alpha, \beta, \gamma ]$, where $\alpha, \beta, \gamma$ are arbitrary real numbers. Note that we exclude mentioning corpus $C$ in both sides of Equation~\ref{eqn:composite} to simplify the set of notations used in this section.

The weight parameters ($\theta$) are {\em tuned adaptively} for a new bug report $b$ based on a set of top-K historical fixed bugs in a training data that are the most similar to $b$. We find these top-K nearest neighbors by measuring the textual similarity of $b$ with training (historical) bug reports using the VSM model. In this work, we propose a probabilistic learning approach which analyzes this training data to fine-tune the weight parameters $\alpha$, $\beta$, and $\gamma$ for the new bug report $b$.

\paragraph{Probabilistic Formulation} \hspace{0pt} 
From a machine learning standpoint, bug localization can be interpreted as a \emph{binary classification} task. For a given combination $(b, p, m)$, the positive label refers to the case when method $m$ is indeed where the bug $b$ is located (i.e., faulty case), and the negative label is when $m$ is not relevant to $b$ (i.e., non-faulty case). As we deal with binary classification task, it is plausible to assume that a data instance follows Bernoulli distribution, c.f.,~\cite{Murphy12}:
\begin{align}
p(x_i, y_i| \theta) &= \sigma(f(x_i, \theta))^{y_i} \left( 1 - \sigma(f(x_i, \theta)) \right)^{(1 - y_i)}
\end{align}

\noindent where $y_i = 1$ ($y_i = 0$) denotes the positive (negative) label, and $\sigma(x) = \frac{1}{1 + \exp(-x)}$ is the logistic function. Using this notation, we can formulate the overall data \emph{likelihood} as:
\begin{align}
\label{eqn:likelihood}
p(X, y | \theta) &= \prod_{i=1}^N \sigma(f(x_i, \theta))^{y_i} \left( 1 - \sigma(f(x_i, \theta)) \right)^{(1 - y_i)}
\end{align}

\noindent where $N$ is the total number of data instances (i.e., $(b,p,m)$ combinations), and $y = [y_1,\ldots,y_i,\ldots,y_N]$ is the label vector.

Our primary interest here is to infer the \emph{posterior} probability $p(\theta | X)$, which can be computed via the Bayes' rule:
\begin{align}
p(\theta | X, y) &= \frac{p(X, y | \theta) p(\theta)}{p(X, y)}
\end{align}

\noindent Specifically, our goal is to find an optimal parameter vector $\theta^{*}$ that maximizes the posterior $p(\theta | X, y)$. This leads to the following optimization task:
\begin{align}
\label{eqn:MAP}
\theta^{*} &= \arg \max_{\theta} p(\theta | X, y) \nonumber\\
&= \arg \max_{\theta} p(X, y | \theta) p(\theta) \nonumber\\
&= \arg \min_{\theta} \left( -\log(p(X, y | \theta)) - \log(p(\theta)) \right)
\end{align}

\noindent Here we can drop the denominator $p(X, y)$, since it is independent of the parameters $\theta$. The term $p(\theta)$ refers to the \emph{prior}, which we define to be a Gaussian distribution with (identical) zero mean and inverse variance $\lambda$:
\begin{align}
\label{eqn:prior}
p(\theta) = \prod_{j=1}^J \sqrt{ \frac{\lambda}{2 \pi} } \exp \left( -\frac{\lambda}{2} \theta_j^2 \right)
\end{align}

\noindent where the number of parameters $J$ is $3$ in our case (i.e., $\alpha$, $\beta$, and $\gamma$).

By substituting (\ref{eqn:likelihood}) and (\ref{eqn:prior}) into (\ref{eqn:MAP}), and by droppping the constant terms that are independent of $\theta$, the optimal parameters $\theta^{*}$ can be computed as:
\begin{align}
\theta^{*} &= \arg \min_{\theta} \left( \sum_{i=1}^N \mathcal{L}_i + \frac{\lambda}{2} \sum_{j=1}^J \theta_j^2 \right)
\end{align}

\noindent where $\mathcal{L}_i$ is called the instance-wise loss, as given by:
\begin{align}
\label{eq:instance-wise-loss}
\mathcal{L}_i = -\left[ y_i \log(\sigma(f(x_i, \theta))) + (1 - y_i) \log(1 - \sigma(f(x_i, \theta))) \right]
\end{align}

\noindent Solution to this minimization task is known as the \emph{regularized logistic regression}. The regularization term $\frac{\lambda}{2} \sum_{j=1}^J \theta_j^2$--which stems from the prior $p(\theta)$--serves to penalize large parameter values, thereby reducing the risk of data overfitting.

\paragraph{Algorithm} \hspace{0pt} 
To estimate $\theta^{*}$, we develop an iterative parameter tuning strategy that performs a descent move along the negative gradient of $\mathcal{L}_i$. Algorithm 1 summarizes our proposed parameter tuning method. More specifically, for each instance $i$, we perform gradient descent update for each parameter $\theta_j$:
\begin{align}
\theta_j \leftarrow \theta_j - \eta \left( \frac{\partial \mathcal{L}_i}{\partial \theta_j} + \lambda \theta_j \right)
\end{align}

\noindent where the gradient term $\frac{\partial \mathcal{L}_i}{\partial \theta_j}$ resolves to:
\begin{align}
\frac{\partial \mathcal{L}_i}{\partial \theta_j} &= \left( \sigma(f(x_i, \theta)) - y_i \right) x_{i,j}
\end{align}

\noindent with the feature values $x_{i,1} = \text{AML}^\text{Text}(b,m)$, $x_{i,2} = \text{AML}^\text{Spectra}(p,m)$ and $x_{i,3} = \text{AML}^\text{SuspWord}(b,p,m)$, corresponding to the parameters $\alpha$, $\beta$ and $\gamma$, respectively. The update steps are realized in lines 11-13 of Algorithm 1.

One key challenge in the current bug localization task is the extremely skewed distribution of the labels, i.e., the number of positive cases is much smaller than the number of negative cases. To address this, we devise a \emph{balanced random sampling} procedure when picking a data instance for gradient descent update. In particular, for every update step, we alternatingly select a random instance from the positive and negative instance pools, as per lines 4-8 of Algorithm 1.

\begin{algorithm}[!t]
\begin{algorithmic}[1]
\Require Matrix $X \in \mathbb{R}^{N \times 3}$ (each row is a vector $x_i = [\text{AML}^{\text{Text}}(b,m), \text{AML}^{\text{Spectra}}(p,m), \text{AML}^{\text{SuspWord}}(b,p,m)]$ for bug report $b$, program spectra $p$, and method $m$ in one of the top-K most similar training data), label vector $y \in \mathbb{R}^{N}$ (each element $y_i$ is the label of $x_i$), learning rate $\eta$, regularization parameter $\lambda$, maximum training iterations $T_{max}$
\Ensure Weight parameters $\alpha$, $\beta$, $\gamma$
\State Initialize $\alpha$, $\beta$, $\gamma$ to zero
\Repeat
	\For {each $n \in \{ 1,\ldots,N \}$}
		\If{$n\bmod{2} = 0$}  \Comment{Draw a positive instance}
			\State{Randomly pick $i$ from $\{1,\ldots,N\}$ s.t. $y_i = 1$}	
		\Else \Comment{Draw a negative instance}
			\State{Randomly pick $i$ from $\{1,\ldots,N\}$ s.t. $y_i = 0$}
		\EndIf
		\State Compute overall score $f(x_i, \theta)$ using Eq. (\ref{eqn:composite})
		\State Compute gradient $g_i \leftarrow \sigma(f(x_i, \theta)) - y_i$
		\State $\alpha \leftarrow \alpha - \eta \left( g_i \times \text{AML}^{\text{Text}}(b,m) + \lambda \alpha \right) $
		\State $\beta \leftarrow \beta - \eta \left( g_i \times \text{AML}^{\text{Spectra}}(p,m) + \lambda \beta \right)$
		\State  $\gamma \leftarrow \gamma - \eta \left( g_i \times \text{AML}^{\text{SuspWord}}(b,p,m) + \lambda \gamma \right)$
	\EndFor
\Until $T_{max}$ iterations
\end{algorithmic}
\caption{Adaptive multi-modal bug localization}
\label{alg:adaptive}
\end{algorithm}

Using this simple method, we can balance the training from positive and negative instances, thus effectively mitigating the issue of {\em skewed distribution} in the localization task. It is also worth noting that our iterative tuning procedure is efficient. That is, its time complexity is linear with respect to the number of instances $N$ and maximum iterations $T_{max}$. %In this work, we use a fixed $T_{max} = 10$. 

==> rq3.tex <==
%\begin{figure}[!htb]
%\centering
%
%\includegraphics[scale=0.5]{boxplot.eps}
%\caption{Contribution of $AML^{SPECTRA}$, $AML^{TEXT}$, and $AML^{BOTH}$}
%\label{fig:boxplot}
%\end{figure}

\begin{table}[!htb]
	\caption{Average weights of each component}
	\centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Project} & $\textbf{AML}^\textbf{Text}$ & $\textbf{AML}^{\textbf{SuspWord}}$ & $\textbf{AML}^\textbf{Spectra}$ \\ \hline\hline
AspectJ&-14.25&33.18&1.94\\\hline
Ant&9.14&12.5&1.54\\\hline
Lucene&12.43&25.77&-0.47\\\hline
Rhino&2.79&1.44&1.81\\\hline
    \end{tabular}
    \label{tab:contributions}
\end{table}

%In this research question, we investigate the contributions of $AML^{SPECTRA}$, $AML^{TEXT}$, and $AML^{BOTH}$ to the overall performance of the whole approach. We consider the default setting of $AML$, i.e., $n=20$. Figure~\ref{fig:boxplot} is the box plot showing the distribution of weights assigned to $AML^{SPECTRA}$, $AML^{TEXT}$, and $AML^{BOTH}$ which correspond to the values of $\alpha$, $\beta$, and $\gamma$ respectively. From the figure, we can note that for most bugs, all of the components are given non-zero weights. This shows that each component is important for a good number of bugs. Also, $AML^{BOTH}$ is often given higher weights than the other two components. The median weights given to $AML^{BOTH}$ and $AML^{SPECTRA}$ are the same, however the third quartile of the weights given to $AML^{BOTH}$ is much higher than the third quartile of the weights given to $AML^{SPECTRA}$. The mean of the weights given to $AML^{BOTH}$, $AML^{SPECTRA}$ and $AML^{TEXT}$ are 0.41, 0.32, and 0.27, respectively. 

%In this research question, we investigate the contribution of $\text{AML}^{\text{Text}}$, $\text{AML}^\text{SuspWord}$, and $\text{AML}^\text{Spectra}$ to the performance of AML in the context of the default setting (i.e., $n=10$). Table~\ref{tab:contributions} highlights the average weights of each AML component in the four projects.  From the Table~\ref{tab:contributions}, $\text{AML}^\text{SuspWord}$ has the highest weights than the other two components in AspectJ, Ant, and Lucene. For Rhino, $\text{AML}^\text{Text}$ has the highest weight (i.e., 2.79). Interestingly, according to Equation~\ref{eqn:composite}, component weights (i.e., $\alpha$, $\beta$, and $\gamma$) can be possible or negative numbers. From the table, AspectJ and Lucene are the two cases have negative component weights. Overall, we find that the component weights are well-tuned to maximize their contributions to the overall AML.

%[say something about the negative weights later ...]
We use default setting of AML ($n=10$) to evaluate contributions of component weights to the effectiveness of  AML. From Equation~\ref{eqn:composite}, we observe that component weights with large absolute values  have stronger influences on final suspiciousness scores of methods (i.e., $f(x_i, \theta)$), and near-zero weights have weaker influences on the suspiciousness scores. Based on our observation and the  result shown in Table~\ref{tab:contributions}, we find that average weights of AML$^\text{Text}$ and AML$^\text{SuspWord}$ in AspectJ, Ant, and Lucene are significantly larger than of AML$^\text{Spectra}$. This implies AML$^\text{Text}$ and AML$^\text{SuspWord}$ have stronger contribution to performance of AML than  AML$^\text{Spectra}$ in AspectJ, Ant, and Lucene. In Rhino, 
AML$^\text{Text}$ has the largest average weight, and AML$^\text{SuspWord}$ has the smallest weight. However, their differences are not significant compared to their magnitudes. Therefore, contributions of the three components to AML in Rhino are  relatively equivalent. On the other hand, AML$^\text{Text}$ and AML$^\text{Spectra}$ have negative average weights in AspectJ and Lucene, respectively. From Equation~\ref{eqn:composite}, we  observe that the purpose of negative weights is to decrease suspiciousness scores of methods when their magnitudes are much larger from the actual suspiciousness. Therefore, negative weights of SW$^\text{Text}$ and AML$^\text{Spectra}$ are for adjusting suspiciousness scores of methods to converge their actual values as much as possible.

==> rq4.tex <==
%\begin{table}[t]
%	\centering
%	\caption{Adaptive vs. Non-Adaptive}
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline
%      \textbf{Setting}& {\textbf{SR@1}} &\textbf{SR@5} &\textbf{SR@10} & \textbf{MAP} \\
%    \hline
%      \textbf{Adaptive} &{17.83\%}&{43.95\%}&{54.78\%}&\multirow{2}{*}{0.218}\\
%    ($AML$)   &(28)&(69)&(86)&\\\hline
%  \textbf{Non-Adaptive} &{???\%}&{???\%}&{???\%}&\multirow{2}{*}{???}\\
%	     ($AML_{*}$)  &(???)&(???)&(???)&\\\hline
%
%    
%    \end{tabular}
%    \label{tab:non_adaptive}
%\end{table}


\begin{table}[t]
	\centering
	\caption{Adaptive vs. non-adaptive learning}
	\scalebox{0.95}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
      \textbf{Project}& \textbf{Setting}&{\textbf{SR@1}} &\textbf{SR@5} &\textbf{SR@10} & \textbf{MAP} \\
    \hline
    \multirow{3}{*}{AspectJ} &$n=20$& 14.63\%&24.39\%&29.27\%&0.163   \\
    &$n=35$&19.51\%&26.83\%&31.71\%&0.199\\ 
    &$AML_{*}$&19.51\%&26.83\%&31.71\%&0.197\\\hline
     \multirow{3}{*}{Ant}  &$n=20$  &15.09\%&39.62\%&58.49\%&0.220 \\ 
&  $n=35$  &16.98\%&43.40\%&58.49\%&0.248\\
        &$AML_{*}$&13.21\%&41.51\%&58.49\%&0.228\\\hline
 \multirow{3}{*}{Lucene}& $n=20$ &29.73\%&64.86\%&75.68\%&0.284  \\ 
&$n=35$ &29.73\%&62.16\%&70.27\%&0.280\\
        &$AML_{*}$&29.73\%&62.16\%&70.27\%&0.280\\\hline
    \multirow{3}{*}{Rhino}&$n=20$   &11.54\%&53.85\%&57.69\%&0.204\\
    &$n=35$ &11.54\%&53.85\%&53.85\%&0.199\\
     & $AML_{*}$   &11.54\%&53.85\%&53.85\%&0.199\\\hline
    \textbf{ \multirow{3}{*}{Overall}}& $n=20$&17.83\%&43.95\%&54.78\%&0.218 \\
   
    &$n=35$ &19.75\%&45.22\%&53.50\%&0.234\\ 
      &$AML_{*}$ &18.47\%&44.59\%&53.50\%&0.227\\\hline
    \end{tabular}}
    \label{tab:non_adaptive}
\end{table}

==> rq6_analysis.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.55\textwidth]{bug_high_crop}
\caption{The proposed NetML framework}
\label{fig:bug_high}
\end{figure}

==> rq_statssig.tex <==
%Table \ref{tab:result_top_N} shows the results of Wilcoxon signed-rank test of AML* and AML among Top N. ($*$) means that results of AML* and AML are significant. AML* and AML are statistically significant in terms of top 1 methods among AspectJ, Ant, and Rhino at significant level 0.05 of Wilcoxon signed-rank test. Moreover, we see that AML* and AML show significant results among all the four software projects in the top 1 methods. Among top 5 methods, only AML* and AML are only significant in project Rhino. In the top 10 methods, AML* and AML do not show any significant results in all software projects. 
%
%Table \ref{tab:result_map} presents the Wilcoxon signed-rank test of AML* and AML in terms of MAP. Similar to top 1 methods, AML* and AML are significant in AspectJ, Ant and Rhino, however they are not significant in project Lucene. However, both methods are significant across four different software data. 

==> time_analysis.tex <==
%Table~\ref{tab:running_time} shows means and standard deviations of AML's running time for different projects. From the table, we note that AML has an average running time of 46.01 seconds. Among the four projects, AML can process Rhino bugs with the least average running time (i.e., 17.94 seconds), and AML needs the longest running time to process AspectJ bugs (i.e., 72.79 seconds). Compared to the other three projects, AspectJ is considerably larger. Therefore, it takes more time for AML to tune its component weights. Considering that a developer can spend hours and even days to fix a bug~\cite{KimW06}, AML running time of 20-80 seconds is reasonable.
%
%
%\begin{table}[t]
%	\caption{Running Time of AML (seconds)}
%	\centering
%    \begin{tabular}{|l|c|c|}
%    \hline
%    \textbf{Project} & \textbf{Mean} & \textbf{Standard Deviation }\\ \hline
%    \hline
%AspectJ&72.79&5.50\\\hline
%Ant&40.88&2.52\\\hline
%Lucene&43.39&3.40\\\hline
%Rhino&17.94&1.58\\\hline
%\hline
%\textbf{Overall}&46.01&18.48\\\hline
%    \end{tabular}
%    \label{tab:running_time}
%\end{table} 
